Scalable Data Notarization Leveraging Hybrid DLTs

Notarization is a procedure that enhance data management by ensuring the authentication of data during audits, thereby increasing trust in the audited data. Blockchain is frequently used as a secure, immutable, and transparent storage, contributing to make data notarization procedures more effective and trustable. Several blockchain-based data notarization protocols have been proposed in literature and commercial solutions. However, these implementations, whether on public or private blockchains, face inherent challenges: high fees on public blockchains and trust issues on private platforms, limiting the adoption of blockchains for data notarization or forcing several trade-offs. In this paper, we explore the use of hybrid blockchain architectures for data notarization, with a focus on scalability issues. Through the analysis of a real-world use case, the data notarization of product passports in supply chains, we propose a novel approach utilizing a data structure designed to efficiently manage the trade-offs in terms of storage occupation and costs involved in notarizing a large collection of data.

==> 2.appoggio.tex <==
Authenticated data structures \cite{tamassia2003Authenticated} allows to proof the data authenticity and integrity. There are several scenarios in which authenticated data structures are successfully applied, with the case of the data replication \cite{devanbu2000authenticated} and data outsourcing \cite{papamanthouT20072parties} as the most well known. In such scenarios, an user could query an untrusted data source (data outsourcing) or an untrusted intermediate third party which manages data from a trusted source (data replication). To address the lack of trust in the data source or in the intermediaries, authenticated data structure are used to generate proof of integrity and/or authenticity about the query result.






In our scenario, we will consider an hybrid DLT architecture, more specifically the one proposed in \cite{hybridDlt}. In this architecture, the operative environment is private, resembling to a private DLT, in which authorized users join and produces new data and interact with the existing ones. This private environment periodically notarizes such data on a public blockchain, in order to make them tamper-proof and publicly verifiable.









Data in the private network are maintained into data structures called \textit{ledgers}, which are made by a series of data blocks chained by hash pointers, similarly to a blockchain ledger. Every ledger has a list of authorized users, which hold a copy of the ledger and can interact with it adding, removing or updating data. Anytime the ledger is updated, other users synchronize their local copies. An intermediate module, the \textit{Notary}, is responsible to handle the updates and keep trace of every ledger history in a dedicated storage. This version of the ledger can be considered as the official one, which all the local copies should refer to. Anytime an user modifies a ledger, they send an update request to the Notary, which updates the official copy and communicates to the other users the update. The Notary is also responsible to manage the notarization of the ledgers on the public blockchain. 

\item \textbf{Tamper-proofness:} the entire notarization process should contribute to ensure that the notarized data have not been tampered with;
   
\item \textbf{Privacy preservation:} the data notarization should support privacy-preserving audits from outside the private network. This implies that an external auditor should have a full access to the compact notarized data, which should be tamper-proof, supported by an eventual more restricted access to the extended data in the private environment.

\item \textbf{External auditability:} the audit of a private DLT by an external auditor, i.e., an auditor which is not part of the private network, can suffer of trust issues. Considering that in a private DLT members are known each other, it is easier to eventually manipulate the consensus in order to create "artificial" data for the auditor, which may not correspond to the real state of the network. In this sense, the notarized data have to act as a support to verify the correctness of the provided data, for both internal and external, at any time. This requirement is trivial to satisfy for internal auditors, considering that they have full access to the entire ledger data. On the other hand, it is possible that an external auditor does not access the entire ledger, but only a selective disclosure of it. In both cases, notarized data should be used to verify that the exported data satisfy some crucial integrity properties, such as data consistency and tamper-proofness;







With this framework, we are able to satisfy the requirements analyzed in Section \ref{sec:problem}: the daily write contributes to create a consistent digest sequence, and the choice of Algorand as public blockchain helps to keep the costs reasonable, because of the low fees and the low block creation time. Moreover, the notarization of only a small digest, instead of an entire data structure, optimizes the space occupation. Algorand transaction structure play a key role in the storage occupation optimization: considering that every transaction offer a free space of 1 kB for notes, the digest can be stored in this note field without the need to use additional storages. Furthermore, the cryptographical digests and the possibility to selectively disclose the ledger data preserves the privacy and also enables external audits. The sequence of digests and the corresponding consistency proofs ensure the tamper-proofness. Finally, the combination of the transparency provided by anchoring on a public blockchain and the security provided by the periodical notarization and by the usage of cryptography to calculate digests and proofs creates the perfect setup to have trustable and privacy-preserving external audits.







First, consistency proofs are related to the entire ledger population. It is not possible to disclose the consistency proof for a single ledger in the tree, the total population has to be accounted.

Then, it is not possible to store the entire data structure on the blockchain. This implies that the proofs cannot be verified independently, but the verification requires some off-chain data. Despite this, the properties of tamper-proofness and consistency are guaranteed by how the notarization and the proof system is implemented. 

Finally, in order to take an acceptable trade-off on proof size, it is not possible to assess that the properties certified by a proof for a specific time moment will hold for more recent time moments. In other terms, given two chronologically order data structure instances identified by the digests $R_1$ and $R_2$ (with $R_2 > R_!$ chronologically), if $R_1$ is tamper-proof and consistent with a $R_0 < R_1$ digest, there are no guarantee that the same proofs guarantee the same properties also for $R_2$. Proofs have to be re-verified, accessing to the current version of the data structure (recall that such data are publicly available, but stored off-chain).

